Baryon Number Dirac Spectrum in QCD

The relation between the baryon number in QCD at nonzero chemical potential and the spectral density of the baryon number Dirac operator, $\gamma_0(D+m)$, is examined. We show that extreme oscillations of the spectral density, caused by the QCD sign problem, are essential for the formation of the average baryon number when $\mu>m_\pi/2$. We compute the oscillating region of the spectral density using chiral perturbation theory. The extreme oscillations have a microscopic period and are resolved using random matrix theory.

==> ref.tex <==
\begin{thebibliography}{99}

%\cite{Banks:1980}
\bibitem{Banks:1980}
  T.~Banks and A.~Casher,
  %``Chiral Symmetry Breaking in Confining Theories,''
  Nucl.\ Phys.\ B {\bf 169} (1980) 103.
  %%CITATION = NUPHA,B169,103;%%

%\cite{Osborn:2005}
\bibitem{Osborn:2005}
  J.~C.~Osborn, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Chiral symmetry breaking and the Dirac spectrum at nonzero chemical potential,''
  Phys.\ Rev.\ Lett.\  {\bf 94} (2005) 202001
  [hep-th/0501210].
  %%CITATION = HEP-TH/0501210;%%

%\cite{Osborn:2008}
\bibitem{Osborn:2008b}
  J.~C.~Osborn, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Chiral Condensate at Nonzero Chemical Potential in the Microscopic Limit of QCD,''
  Phys.\ Rev.\ D {\bf 78} (2008) 065029
  [arXiv:0805.1303 [hep-th]].
  %%CITATION = ARXIV:0805.1303;%%

%\cite{Osborn:2004}
\bibitem{Osborn:2004}
  J.~C.~Osborn,
  %``Universal results from an alternate random matrix model for QCD with a baryon chemical potential,''
  Phys.\ Rev.\ Lett.\  {\bf 93} (2004) 222001
  [hep-th/0403131].
  %%CITATION = HEP-TH/0403131;%%

%\cite{Akemann:2004}
\bibitem{Akemann:2004}
  G.~Akemann, J.~C.~Osborn, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Unquenched QCD Dirac operator spectra at nonzero baryon chemical potential,''
  Nucl.\ Phys.\ B {\bf 712} (2005) 287
  [hep-th/0411030].
  %%CITATION = HEP-TH/0411030;%%

%\cite{Osborn:2005}
\bibitem{XQCD}
  J.~C.~Osborn, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``The Sign problem is the solution,''
  hep-lat/0510118.
  %%CITATION = HEP-LAT/0510118;%%

%\cite{Barbour:1986}
\bibitem{Barbour:1986}
  I.~Barbour, N.~E.~Behilil, E.~Dagotto, F.~Karsch, A.~Moreo, M.~Stone and H.~W.~Wyld,
  %``Problems with Finite Density Simulations of Lattice QCD,''
  Nucl.\ Phys.\ B {\bf 275} (1986) 296.
  %%CITATION = NUPHA,B275,296;%%

\bibitem{Ravagli:2007}
  L.~Ravagli and J.~J.~M.~Verbaarschot,
  %``QCD in One Dimension at Nonzero Chemical Potential,''
  Phys.\ Rev.\ D {\bf 76}, 054506 (2007)
  [arXiv:0704.1111 [hep-th]].
  %%CITATION = ARXIV:0704.1111;%%

\bibitem{Akemann:2011}
  G.~Akemann, T.~Kanazawa, M.~J.~Phillips and T.~Wettig,
  %``Random matrix theory of unquenched two-colour QCD with nonzero chemical potential,''
  JHEP {\bf 1103}, 066 (2011)
  [arXiv:1012.4461 [hep-lat]].
  %%CITATION = ARXIV:1012.4461;%%

%\cite{Gibbs:1986}
\bibitem{Gibbs:1986}
  P.~E.~Gibbs,
  %``Lattice Monte Carlo Simulations Of Qcd At Finite Baryonic Density,''
  Phys.\ Lett.\ B {\bf 182} (1986) 369.
  %%CITATION = PHLTA,B182,369;%%

%\cite{Stephanov:1996}
\bibitem{Stephanov:1996}
  M.~A.~Stephanov,
  %``Random matrix model of QCD at finite density and the nature of the quenched limit,''
  Phys.\ Rev.\ Lett.\  {\bf 76} (1996) 4472
  [hep-lat/9604003].
  %%CITATION = HEP-LAT/9604003;%%

%\cite{Gocksch:1988}
\bibitem{Gocksch:1988}
  A.~Gocksch,
  %``On Lattice Qcd At Finite Density,''
  Phys.\ Rev.\ D {\bf 37} (1988) 1014.
  %%CITATION = PHRVA,D37,1014;%%

%\cite{Osborn:2008}
\bibitem{Osborn:2008}
  J.~C.~Osborn, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Phase Diagram of the Dirac Spectrum at Nonzero Chemical Potential,''
  Phys.\ Rev.\ D {\bf 78} (2008) 105006
  [arXiv:0807.4584 [hep-lat]].
  %%CITATION = ARXIV:0807.4584;%%

%\cite{Osborn:2005b}
\bibitem{Osborn:2005b}
  J.~C.~Osborn, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Chiral symmetry breaking and the Dirac spectrum at nonzero chemical potential,''
  Phys.\ Rev.\ Lett.\  {\bf 94} (2005) 202001
  [hep-th/0501210].
  %%CITATION = HEP-TH/0501210;%%

%\cite{Damgaard:2000}
\bibitem{Damgaard:2000}
  P.~H.~Damgaard and K.~Splittorff,
  %``Partially quenched chiral perturbation theory and the replica method,''
  Phys.\ Rev.\ D {\bf 62} (2000) 054509
  [hep-lat/0003017].
  %%CITATION = HEP-LAT/0003017;%%

%\cite{Gasser:1984}
\bibitem{Gasser:1984} 
  J.~Gasser and H.~Leutwyler,
  %``Chiral Perturbation Theory to One Loop,''
  Annals Phys.\  {\bf 158}, 142 (1984).
  %%CITATION = APNYA,158,142;%%

%\cite{Gasser:1985}
\bibitem{Gasser:1985} 
  J.~Gasser and H.~Leutwyler,
  %``Chiral Perturbation Theory: Expansions in the Mass of the Strange Quark,''
  Nucl.\ Phys.\ B {\bf 250}, 465 (1985).
  %%CITATION = NUPHA,B250,465;%%

%\cite{Pich:1998}
\bibitem{Pich:1998}
  A.~Pich,
  %``Effective field theory: Course,''
  hep-ph/9806303.
  %%CITATION = HEP-PH/9806303;%%

%\cite{Son:2000}
\bibitem{Son:2000}
  D.~T.~Son and M.~A.~Stephanov,
  %``QCD at finite isospin density,''
  Phys.\ Rev.\ Lett.\  {\bf 86} (2001) 592
  [hep-ph/0005225].
  %%CITATION = HEP-PH/0005225;%%

%\cite{GellMann:1968}
\bibitem{GellMann:1968}
  M.~Gell-Mann, R.~J.~Oakes and B.~Renner,
  %``Behavior of current divergences under SU(3) x SU(3),''
  Phys.\ Rev.\  {\bf 175} (1968) 2195.
  %%CITATION = PHRVA,175,2195;%%

%\cite{Halasz:1997}
\bibitem{Halasz:1997}
  A.~M.~Halasz, A.~D.~Jackson and J.~J.~M.~Verbaarschot,
  %``Fermion determinants in matrix models of QCD at nonzero chemical potential,''
  Phys.\ Rev.\ D {\bf 56} (1997) 5140
  [hep-lat/9703006].
  %%CITATION = HEP-LAT/9703006;%%

%\cite{Halasz:1999}
\bibitem{Halasz:1999} 
  A.~M.~Halasz, J.~C.~Osborn, M.~A.~Stephanov and J.~J.~M.~Verbaarschot,
  %``Random matrices and the convergence of partition function zeros in finite density QCD,''
  Phys.\ Rev.\ D {\bf 61}, 076005 (2000)
  [hep-lat/9908018].
  %%CITATION = HEP-LAT/9908018;%%

%\cite{Kogut:2001}
\bibitem{Kogut:2001}
  J.~B.~Kogut and D.~Toublan,
  %``QCD at small nonzero quark chemical potentials,''
  Phys.\ Rev.\ D {\bf 64} (2001) 034007
  [hep-ph/0103271].
  %%CITATION = HEP-PH/0103271;%%

%\cite{Verbaarschot:1985}
\bibitem{Verbaarschot:1985}
  J.~J.~M.~Verbaarschot and M.~R.~Zirnbauer,
  %``Critique of the Replica Trick,''
  J.\ Phys.\ A A {\bf 18} (1985) 1093.
  %%CITATION = JPAGB,A18,1093;%%

\bibitem{Zirnbauer:2003}
  M.~R.~Zirnbauer,
  arXiv:cond-mat/9903338.

%\cite{Akemann:2007}
\bibitem{Akemann:2007}
  G.~Akemann,
  %``Matrix Models and QCD with Chemical Potential,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 22} (2007) 1077
  [hep-th/0701175].
  %%CITATION = HEP-TH/0701175;%%

%\cite{Ginibre:1965}
\bibitem{Ginibre:1965}
  J.~Ginibre,
  %``Statistical Ensembles of Complex, Quaternion and Real Matrices,''
  J.\ Math.\ Phys.\  {\bf 6} (1965) 440.
  %%CITATION = JMAPA,6,440;%%

%\cite{Akemann:2002}
\bibitem{Akemann:2002}
  G.~Akemann and G.~Vernizzi,
  %``Characteristic polynomials of complex random matrix models,''
  Nucl.\ Phys.\ B {\bf 660} (2003) 532
  [hep-th/0212051].
  %%CITATION = HEP-TH/0212051;%%

%\cite{Akemann:2004b}
\bibitem{Akemann:2004b}
  G.~Akemann, Y.~V.~Fyodorov and G.~Vernizzi,
  %``On matrix model partition functions for QCD with chemical potential,''
  Nucl.\ Phys.\ B {\bf 694} (2004) 59
  [hep-th/0404063].
  %%CITATION = HEP-TH/0404063;%%

\bibitem{Sharpe+}
  S.~R.~Sharpe and R.~L.~Singleton, Jr,
  %``Spontaneous flavor and parity breaking with Wilson fermions,''
  Phys.\ Rev.\ D {\bf 58} (1998) 074501
  [hep-lat/9804028].
  %%CITATION = HEP-LAT/9804028;%%
  G.~Rupak and N.~Shoresh,
  %``Chiral perturbation theory for the Wilson lattice action,''
  Phys.\ Rev.\ D {\bf 66} (2002) 054503
  [hep-lat/0201019].
  %%CITATION = HEP-LAT/0201019;%%
  O.~Bar, G.~Rupak and N.~Shoresh,
  %``Chiral perturbation theory at O(a**2) for lattice QCD,''
  Phys.\ Rev.\ D {\bf 70} (2004) 034508
  [hep-lat/0306021].
  %%CITATION = HEP-LAT/0306021;%%
  S.~R.~Sharpe and J.~M.~S.~Wu,
  %``The Phase diagram of twisted mass lattice QCD,''
  Phys.\ Rev.\ D {\bf 70} (2004) 094029
  [hep-lat/0407025].
  %%CITATION = HEP-LAT/0407025;%%
  M.~Golterman, S.~R.~Sharpe and R.~L.~Singleton, Jr.,
  %``Effective theory for quenched lattice QCD and the Aaoki phase,''
  Phys.\ Rev.\ D {\bf 71} (2005) 094503
  [hep-lat/0501015].
  %%CITATION = HEP-LAT/0501015;%%

%\cite{Akemann:2010}
\bibitem{Akemann:2010}
  G.~Akemann, P.~H.~Damgaard, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Spectrum of the Wilson Dirac Operator at Finite Lattice Spacings,''
  Phys.\ Rev.\  D {\bf 83} (2011) 085014
  [arXiv:1012.0752 [hep-lat]].
  %%CITATION = PHRVA,D83,085014;%%

%\cite{Damgaard:2010}
\bibitem{Damgaard:2010}
  P.~H.~Damgaard, K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Microscopic Spectrum of the Wilson Dirac Operator,''
  Phys.\ Rev.\ Lett.\  {\bf 105} (2010) 162002
  [arXiv:1001.2937 [hep-th]].
  %%CITATION = ARXIV:1001.2937;%%

%\cite{Damgaard:1999}
\bibitem{Damgaard:1999}
  P.~H.~Damgaard, J.~C.~Osborn, D.~Toublan and J.~J.~M.~Verbaarschot,
  %``The microscopic spectral density of the {QCD} Dirac operator,''
  Nucl.\ Phys.\  B {\bf 547} (1999) 305
  [arXiv:hep-th/9811212].
  %%CITATION = NUPHA,B547,305;%%

%\cite{Feinberg:1997}
\bibitem{Feinberg:1997}
  J.~Feinberg and A.~Zee,
  %``NonHermitian random matrix theory: Method of Hermitean reduction,''
  Nucl.\ Phys.\ B {\bf 504} (1997) 579
  [cond-mat/9703087].
  %%CITATION = COND-MAT/9703087;%%

%\cite{Toublan:1999}
\bibitem{Toublan:1999}
  D.~Toublan and J.~J.~M.~Verbaarschot,
  %``Effective low-energy theories and QCD Dirac spectra,''
  Int.\ J.\ Mod.\ Phys.\ B {\bf 15} (2001) 1404
  [hep-th/0001110].
  %%CITATION = HEP-TH/0001110;%%

%\cite{Toublan:2000}
\bibitem{Toublan:2000}
  D.~Toublan and J.~J.~M.~Verbaarschot,
  %``Statistical properties of the spectrum of the QCD Dirac operator at low-energy,''
  Nucl.\ Phys.\ B {\bf 603} (2001) 343
  [hep-th/0012144].
  %%CITATION = HEP-TH/0012144;%%

%\cite{Damgaard:2006}
\bibitem{Damgaard:2006}
  P.~H.~Damgaard, U.~M.~Heller, K.~Splittorff, B.~Svetitsky and D.~Toublan,
  %``Microscopic eigenvalue correlations in QCD with imaginary isospin chemical potential,''
  Phys.\ Rev.\ D {\bf 73} (2006) 105016
  [hep-th/0604054].
  %%CITATION = HEP-TH/0604054;%%

%\cite{Leutwyler:1992}
\bibitem{Leutwyler:1992}
  H.~Leutwyler and A.~V.~Smilga,
  %``Spectrum of Dirac operator and role of winding number in QCD,''
  Phys.\ Rev.\ D {\bf 46} (1992) 5607.
  %%CITATION = PHRVA,D46,5607;%%

%\cite{Splittorff:2006}
\bibitem{Splittorff:2006}
  K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``QCD with Bosonic Quarks at Nonzero Chemical Potential,''
  Nucl.\ Phys.\ B {\bf 757} (2006) 259
  [hep-th/0605143].
  %%CITATION = HEP-TH/0605143;%%

%\cite{Splittorff:2004}
\bibitem{Splittorff:2004}
  K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Factorization of correlation functions and the replica limit of the Toda lattice equation,''
  Nucl.\ Phys.\ B {\bf 683} (2004) 467
  [hep-th/0310271].
  %%CITATION = HEP-TH/0310271;%%

%\cite{Fyodorov:2002}
\bibitem{Fyodorov:2002}
  Y.~V.~Fyodorov,
  %``Negative moments of characteristic polynomials of random matrices: Ingham-Siegel integral as an alternative to Hubbard-Stratonovich transformation,''
  Nucl.\ Phys.\ B {\bf 621} (2002) 643
  [math-ph/0106006].
  %%CITATION = MATH-PH/0106006;%%

%\cite{Splittorff:2002}
\bibitem{Splittorff:2002}
  K.~Splittorff and J.~J.~M.~Verbaarschot,
  %``Replica limit of the Toda lattice equation,''
  Phys.\ Rev.\ Lett.\  {\bf 90} (2003) 041601
  [cond-mat/0209594].
  %%CITATION = COND-MAT/0209594;%%

\bibitem{Andreev:1994}
  A.~V.~Andreev, B.~D.~Simons and N.~Taniguchi
  %``Supersymmetry applied to the spectrum edge of random matrix ensembles,''
  Nucl.\ Phys.\ B {\bf 432} (1994) 487


\end{thebibliography}
